Imitating Unknown Policies via Exploration

Behavioral cloning is an imitation learning technique that teaches an agent how to behave through expert demonstrations. Recent approaches use self-supervision of fully-observable unlabeled snapshots of the states to decode state-pairs into actions. However, the iterative learning scheme from these techniques are prone to getting stuck into bad local minima. We address these limitations incorporating a two-phase model into the original framework, which learns from unlabeled observations via exploration, substantially improving traditional behavioral cloning by exploiting (i) a sampling mechanism to prevent bad local minima, (ii) a sampling mechanism to improve exploration, and (iii) self-attention modules to capture global features. The resulting technique outperforms the previous state-of-the-art in four different environments by a large margin.

==> Imitating Unknown Policies/algo/algorithm.tex <==
\begin{algorithm}[!hbt]
    % \scriptsize
    \caption{High-level IUPE framework.}
    \begin{algorithmic}[1]
        \State Initialize model $\mathcal{M}_\theta$ as a random approximator
        \State Initialize policy $\pi_\phi$ with random weights
        \State Generate $\mathcal{I}^{pre}$ using policy $\pi_\phi$
        \State Generate state transitions $\Tau^{e}$ from demonstrations $D$
        \State Set $\mathcal{I}^s = \mathcal{I}^{pre}$
        \State Let $\alpha$ be the number of improvement cycles
        \For { $i \gets 0$ to $\alpha$ }
            \State Improve $\mathcal{M}_{\theta}$ by trainIDM($\mathcal{I}^s$)
            \State Use $\mathcal{M}_{\theta}$ with $\Tau^{e}$ to predict actions $\hat{A}$
            \State Improve $\pi_\phi$ by behavioralCloning($\Tau^{e}$, $\hat{A}$)
            
            \For { $e \gets 1$ to $\left|E\right|$ }
                \State Use $\pi_\phi$ to solve environment $e$ 
                \State Append samples $\mathcal{I}^{pos} \gets (s_t, \hat{a}_t, s_{t+1})$
                \If { $\pi_\phi$ at goal $g$}
                    \State Append $v_e \gets 1$
                \Else 
                    \State Append $v_e \gets 0$
                \EndIf
            \EndFor
            \State Set $\mathcal{I}^s =$ sampling($\mathcal{I}^{pre}$, $\mathcal{I}^{pos}$, $P(g|E)$, $v_e$)
        \EndFor
    \end{algorithmic}
    \label{alg:iupe}
\end{algorithm}

==> Imitating Unknown Policies/tables/ablation.tex <==
\begin{table}[!t]
    \centering
    \scriptsize
    \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrr} 
        \toprule
        Model & $P$ & $AER$ \\ 
        \midrule
        BCO                                       & $-0.416$         &  $-0.941$ \\
        Attention                                 & $-0.415$         &  $-0.940$ \\
        Sampling                                  & $0.534$          &  $0.348$ \\
        Exploration                               & $0.734$          &  $0.605$ \\
        Attention + Sampling                      & $0.367$          &  $0.088$ \\ 
        Attention + Exploration                   & $-0.407$         &  $-0.921$ \\
        Sampling + Exploration                    & $0.943$          &  $0.901$ \\
        Attention + Sampling + Exploration (IUPE) & $\mathbf{1.000}$ &  $\mathbf{0.981}$ \\ 
        \bottomrule
    \end{tabular*}
    \caption{Ablation study considering IUPE's 3 main components in the maze environment.}
    \label{tab:ablation}
\end{table}

==> Imitating Unknown Policies/tables/results.tex <==
\begin{table*}[tb!]
  \centering
  \scriptsize
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} c c  r r r r r r}
    \toprule
        \multicolumn{1}{c}{Models} & \multicolumn{1}{c }{Metrics} & CartPole & Acrobot & MountainCar & Maze $3\times3$ & Maze $5\times5$ & Maze $10\times10$\\
    
    \midrule
    
    \multirow{2}{*}{Expert} 
     & $P$                       & $1.000$   & $1.000$ & $1.000$ & $1.000$ & $1.000$ & $1.000$\\
     & $AER$                     & $442.628$ & $-110.109$ & $-147.265$ & $0.963$ & $0.970$ & $0.981$\\
    \midrule
    
    \multirow{2}{*}{Random} 
     & $P$                       & $0.000$  & $0.000$    & $0.000$    & $0.000$ & $0.000$ & $0.000$\\
     & $AER$                     & $18.700$ & $-482.600$ & $-200.000$ & $0.557$ & $0.166$ & $-0.415$\\
    
    \midrule

    \multirow{2}{*}{BC} 
     & $P$                       & $1.135$   & $1.071$   &  $1.560$   & $-1.207$ & $-0.921$ & $-0.470$\\
     & $AER$                     & $500.000$ & $-83.590$ & $-117.720$ & $0.180$  & $-0.507$ & $-1.000$\\
    
\midrule
\midrule
    
    \multirow{2}{*}{BCO}
     & $P$                       & $\mathbf{1.135}$   & $0.980$    & $0.948$    & $0.883$ & $-0.112$ & $-0.416$\\
     & $AER$                     & $\mathbf{500.000}$ & $-117.600$ & $-150.000$ & $\mathbf{0.927}$ & $0.104$  & $-0.941$\\
    \midrule
    
    \multirow{2}{*}{ILPO}  
     & $P$                       & $\mathbf{1.135}$   & $1.067$   &	$0.626$	& $-1.711$ & $-0.398$ &	$0.257$\\
     & $AER$                     & $\mathbf{500.000}$ & $-85.300$ & $-167.000$ & $-0.026$ & $-0.059$ & $-0.020$\\
    \midrule
    
    \multirow{2}{*}{IUPE} 
     & $P$                       & $\mathbf{1.135}$   & $\mathbf{1.086}$   & $\mathbf{1.314}$    & $\mathbf{1.361}$ & $\mathbf{1.000}$ & $\mathbf{1.000}$\\
     & $AER$                     & $\mathbf{500.000}$ & $\mathbf{-78.100}$ & $\mathbf{-130.700}$ & $\mathbf{0.927}$ & $\mathbf{0.971}$ & $\mathbf{0.981}$\\
    \bottomrule
\end{tabular*}
\caption{\emph{Performance} and \emph{Average Episode Reward} for our approach and related work.}
\label{tab:results}
\end{table*}
